Rectifying Administrated ERC20 Tokens

The developers of Ethereum smart contracts often implement administrating patterns, such as censoring certain users, creating or destroying balances on demand, destroying smart contracts, or injecting arbitrary code. These routines turn an ERC20 token into an administrated token - the type of Ethereum smart contract that we scrutinize in this research. We discover that many smart contracts are administrated, and the owners of these tokens carry lesser social and legal responsibilities compared to the traditional centralized actors that those tokens intend to disrupt. This entails two major problems: a) the owners of the tokens have the ability to quickly steal all the funds and disappear from the market; and b) if the private key of the owner's account is stolen, all the assets might immediately turn into the property of the attacker. We develop a pattern recognition framework based on 9 syntactic features characterizing administrated ERC20 tokens, which we use to analyze existing smart contracts deployed on Ethereum Mainnet. Our analysis of 84,062 unique Ethereum smart contracts reveals that nearly 58% of them are administrated ERC20 tokens, which accounts for almost 90% of all ERC20 tokens deployed on Ethereum. To protect users from the frivolousness of unregulated token owners without depriving the ability of these owners to properly manage their tokens, we introduce SafelyAdministrated - a library that enforces a responsible ownership and management of ERC20 tokens. The library introduces three mechanisms: deferred maintenance, board of trustees and safe pause. We implement and test SafelyAdministrated in the form of Solidity abstract contract, which is ready to be used by the next generation of safely administrated ERC20 tokens.

==> discussion.tex <==
\section{Limitation}\label{sec:discussion}
One limitation of \emph{SafelyAdministrated} is that the trustee whose vote attains the voting threshold effectively pays fees for the execution of the maintenance transaction, while other trustees pay only for execution of recording of their vote. Although we assume that this unfairness is unlikely to be important in most cases, we leave the implementation of fee reimbursement for future work.

